BORWin: Exact algorithm based on a Bi-Objective Relaxation for Window-constrained problems

A mixed integer maximization problem involving several additional constraints defined with both a lower and an upper bound is considered. It is assumed that one of such constraints is more restrictive than the others. As it can be seen as a resource window constraint, it defines the so-called window-constrained problem. From a bi-objective perspective, a 2-phase algorithm, called BORWin, is devised. It stands for Bi-Objective Relaxation for Window-constrained problems. The first phase is generic for any window-constrained problem and provides a family of upper bounds based on a bi-objective relaxation of the additional constraints. It is shown that the latter bounds strongly relate to the Lagrangian dual bounds. The second phase is derived for a variant involving a graph structure, namely the window-constrained longest-path problem on an acyclic graph. The aim is to take advantage of the upper bounds to devise an efficient label extension algorithm. It is shown that complementary upper bounds could be derived to further improve performance in some special cases. A typical example is when the additional constraints have special knapsack structures. This is the case for the Hydro-Unit Commitment problem with a single plant (1-HUC). From numerical experiments for the 1-HUC, BOR-Win appears to be very efficient compared to state-of-the-art approaches.

==> newsections/algo_old_12012025.tex <==
\section{Phase I of the BORWin algorithm: bi-objective relaxation upper bounds}
\label{sec:phase1}

In this section, we present the first phase of the Bi-Objective relaxation of Resource Windows (BORWin) algorithm, which consists in computing a family of upper bounds for $(P)$ based on the considered bi-objective relaxation \CR{$(BOR)$}.
This bi-objective relaxation is presented in details in Section \ref{sec:borel}.
The properties yielding the family of upper bounds and the tightest of them are established in Section \ref{familyub}. The first-phase algorithm is presented in Section \ref{sec:exfirstphase}.

\subsection{Bi-objective relaxation}
\label{sec:borel}

The idea of the bi-objective relaxation is the following :  additional constraints \eqref{additional_constraints} are relaxed, and the main additional constraint \eqref{main_additional_constraint} is turned into an optimization criterion.

To do so, consider an optimal solution $x^*_{SP}$ of subproblem $(SP)$.
We distinguish 3 cases :
\begin{itemize}
    \item ``Locally Infeasible by Default" (LID), if $\gamma x^*_{SP} < \beta $ 
    \item ``Locally Infeasible by Excess" (LIE), if $\gamma x^*_{SP} > \alpha $
    \item ``Locally Feasible" (LF), otherwise
\end{itemize}
The term ``locally'' means that feasibility is only related to (SP) plus constraint \eqref{main_additional_constraint}. Side-constraints \eqref{additional_constraints} are ignored %at 
in this phase and will be dealt with in the second phase of the method.

Without loss of generality, we suppose in the following that we are in the LID case. 
Therefore, in this section we consider the following relaxation of $(P)$:
\begin{alignat}{3}
     (R) \quad & \underset{x} {\text{max}}
    & & cx \nonumber \\
    & \text{s. t.} \quad
    & & x \in X \nonumber \\
    &&& \beta \leq \gamma x \label{borne_min_ressource}
\end{alignat}

\color{CR}

The results described in this section will rely on the bi-objective relaxation $(BOR)$ of $(R)$, maximizing the vector of objective $cx$ and $\gamma x$.

\color{black}
We denote $\arcvalobj{1}{x} = cx$ and $\arcvalobj{2}{x} = \gamma x$. \vspace{2mm}
\begin{dfn}[Aggregated value]
\color{AH}Consider a vector $\delta=(\delta_1, \delta_2) \in \mathbb{R}^+ $. \color{black}
For a solution $x \in X$, we define $\agg{\delta}{x}=\delta_{1} \cdot \arcvalobj{1}{x}+\delta_{2} \cdot \arcvalobj{2}{x}$ as the aggregated value of a solution $x$ considering vector $\delta$.
\end{dfn}
Note that a solution $x$ is Pareto-supported if there exists a vector $\delta$ such that $\agg{\delta}{x}\geq \agg{\delta}{x'}$ for any other solution $x'$, becase in this case $x$ belongs to the convex hull of the feasible points in the objective space.

\color{AH}
We provide the following definition for the Pareto-equality and Pareto-difference.

\begin{dfn}[Pareto-equality and Pareto-difference definitions]
    Consider two solutions $x$ and $x'$.
    Solutions $x$ and $x'$ are Pareto-equal, denoted $x\paretoeq{} x'$, if $\arcvalobj{1}{x}=\arcvalobj{1}{x'}$ and $\arcvalobj{2}{x}=\arcvalobj{2}{x'}$.
    Otherwise, $x\paretoneq{} x'$. \label{def:Pareto}
\end{dfn}
\color{black}

In the following, we denote $S$ the ordered set of Pareto-supported solutions, ordered by increasing value of the first objective $\arcvalobj{1}{x} = cx$.
We do not consider in $S$ two solutions with the exact same values, meaning that for two solution $x$ and $x'$ in $S$, $x\paretoneq{} x'$.


In this section, we first define some properties for the solutions of $(BOR)$.
Besides, we show that one can obtain a family of upper bounds for $(P)$ using solutions of $(BOR)$ with a well-chosen $\delta$ \color{AH} for their aggregated value. \color{black}
In Section \ref{sec:borwin}, we will use such results to efficiently compute these bounds in the first phase of the BORWin algorithm. The second phase will also exploit these results to restrict the search space.







\subsection{Family of upper-bounds}
\label{familyub}

First, we can introduce an upper bound for $\arcvalobj{1}{x^{*}}$ with $x^{*}$ the optimal solution of (P).

\vspace{2mm}
\begin{pte}
    \label{pte:graphs_twophases:trivial_bound}
    Let $x$ be the Pareto-supported solution maximizing $\arcvalobj{1}{x}$ and $x^{*}$ the optimal solution of (P).
    Then, $\arcvalobj{1}{x}$ is a valid upper bound for $\arcvalobj{1}{x^{*}}$.
\end{pte}
\begin{proof}
    As $x^{*}$ is a valid solution for (P), it is also a valid solution for the (BOR).
    Consequently, if $\arcvalobj{1}{x^{*}}>\arcvalobj{1}{x}$, then $x$ cannot be the Pareto-supported solution maximizing $\arcvalobj{1}{x}$.
    \color{AH}We then deduce $\arcvalobj{1}{x^{*}} \leq \arcvalobj{1}{x}$. \color{black}
\end{proof}
However, it can be possible to provide a tighter upper bound.
We first introduce the following lemma.

\vspace{2mm}
\begin{lem}
    \label{lem:graphs_twophases:not_pareto}
    Let $x_{1}$, $x_{2}$ and $x_{3}$ be three solutions of (BOR) with $\arcvalobj{1}{x_{1}}\leq \arcvalobj{1}{x_{2}}\leq \arcvalobj{1}{x_{3}}$.
    Consider that these solutions do not dominate each other.
    Let $\delta$ be such that $\agg{\delta}{x_{1}}=\agg{\delta}{x_{3}}$.
    If $\agg{\delta}{x_{2}}<\agg{\delta}{x_{1}}$ then $x_{2}$ cannot be Pareto-supported.
\end{lem}
\begin{proof}
    Consider a vector $\delta'$ such that $\delta'_{1}>\delta_{1}$ and $\delta'_{2}=\delta_{2}$.
    Then, as $\agg{\delta}{x_{2}}<\agg{\delta}{x_{3}}$ and $\arcvalobj{1}{x_{2}}\leq \arcvalobj{1}{x_{3}}$, hence $\agg{\delta'}{x_{2}}\leq \agg{\delta'}{x_{3}}$.
    
    Consider a vector $\delta'$ such that $\delta'_{1}<\delta_{1}$ and $\delta'_{2}=\delta_{2}$.
    Then, as $\agg{\delta}{x_{2}}<\agg{\delta}{x_{1}}$ and $\arcvalobj{1}{x_{1}}\leq \arcvalobj{1}{x_{2}}$, hence $\agg{\delta'}{x_{2}}\leq \agg{\delta'}{x_{1}}$.

    From a vector $\delta'$, one can obtain any other vector $\delta''$ by multiplying $\delta'_{1}$ and $\delta'_{2}$ by the same non-negative real number.
    Hence, there is no vector $\delta''$ for which $x_{2}$ maximizes $\agg{\delta''}{x_{2}}$, hence $x_{2}$ is not Pareto-supported by definition.
\end{proof}

We introduce \textbf{Properties \ref{pte:graphs_twophases:valid_upper_bound1}} to \textbf{\ref{pte:graphs_twophases:best_R}} and \textbf{Theorem \ref{thm:graphs_twophases:best_upper_bound}} to provide a tighter upper bound for $\arcvalobj{1}{x^{*}}$.


\vspace{2mm}
\begin{pte}
    \label{pte:graphs_twophases:valid_upper_bound1}
    Let $(x_{1},x_{2})$ be a pair of consecutive solutions in $S$.
    Let $\delta$ be such that $\agg{\delta}{x_{1}}=\agg{\delta}{x_{2}}$.
    For each feasible solution $x_{3}$ of (BOR), $\arcvalobj{1}{x_{3}}\leq \frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot \arcvalobj{2}{x_{3}}}{\delta_{1}}$
\end{pte}

\color{AH}
The proof of \textbf{Property \ref{pte:graphs_twophases:valid_upper_bound1}} is in \textbf{Appendix \ref{anx:graphs_twophases:valid_upper_bound1}}.

\color{black}

\vspace{2mm}
\begin{crl}
    \label{crl:graphs_twophases:valid_upper_bound1}
    Let $(x_{1},x_{2})$ be a pair of solutions in $S$.
    Let $\delta$ be a vector such that $\agg{\delta}{x_{1}}=\agg{\delta}{x_{2}}$.
    Let $x_{3}$ be the solution maximizing $\agg{\delta}{x_{3}}$.
    If solution $x_{3}\paretoneq{} x_{1}$ and $x_{3}\paretoneq{} x_{2}$, then $\arcvalobj{1}{x_{3}} \in ]\arcvalobj{1}{x_{1}};\arcvalobj{1}{x_{2}}[$ and $\arcvalobj{2}{x_{3}} \in ]\arcvalobj{2}{x_{2}};\arcvalobj{2}{x_{1}}[$.
    If solution $x_{3}\paretoeq{} x_{1}$ or $x_{3}\paretoeq{} x_{2}$, then $x_{1}$ and $x_{2}$ are consecutive solutions in S.
\end{crl}
\begin{proof}
    The proof of \textbf{Property \ref{pte:graphs_twophases:valid_upper_bound1}} indicates that if $x_{3}\paretoneq{} x_{1}$ and $x_{3}\paretoneq{} x_{2}$, then $\arcvalobj{1}{x_{3}} \in ]\arcvalobj{1}{x_{1}};\arcvalobj{1}{x_{2}}[$ and $\arcvalobj{2}{x_{3}} \in ]\arcvalobj{2}{x_{2}};\arcvalobj{2}{x_{1}}[$.
    Otherwise, either $x_{1}$ or $x_{2}$ cannot be Pareto-supported, which yields a contradiction.

    In the case $x_{3}\paretoeq{} x_{1}$ or $x_{3}\paretoeq{} x_{2}$, then clearly there cannot be any Pareto-supported solution $x_{4}$ with $\arcvalobj{1}{x_{4}} \in ]\arcvalobj{1}{x_{1}};\arcvalobj{1}{x_{2}}[$ as it cannot be part of the solutions' convex hull in the objective space.
\end{proof}
For a solution $x$ of (BOR), provided we know the value $\arcvalobj{2}{x}$, this property gives an upper bound for $\arcvalobj{1}{x}$ for each pair of consecutive solutions in $S$.
As the optimal solution $x^{*}$ of (P) is also a feasible solution of (BOR), it also applies to $x^{*}$.
As we do not know the value $\arcvalobj{2}{x^{*}}$, we cannot use this property directly.
However, we know that $\arcvalobj{2}{x^{*}}\in [\beta;\alpha]$.

\vspace{2mm}
\begin{pte}
    \label{pte:graphs_twophases:valid_upper_bound2}
    Let $(x_{1},x_{2})$ be a pair of consecutive solutions in $S$.
    Let $\delta$ be such that $\agg{\delta}{x_{1}}=\agg{\delta}{x_{2}}$.
    Let $\bsupvalobj{1}{x_{1}}{\delta}=\frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot \beta}{\delta_{1}}$ be the value on the first objective of the point intersecting the line going through $x_{1}$ with coefficient $\delta$ and the bound $\beta$.
    Then $\bsupvalobj{1}{x_{1}}{\delta}$ is an upper bound for the value of the optimal solution $\arcvalobj{1}{x^{*}}$ of (P).
\end{pte}
\begin{proof}
    As $x^{*}$ is a feasible solution of (P), it is also a feasible solution of (BOR).
    From \textbf{Property \ref{pte:graphs_twophases:valid_upper_bound1}}, we know that $\arcvalobj{1}{x^{*}}\leq \frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot \arcvalobj{2}{x^{*}}}{\delta_{1}}$.
    As $x^{*}$ is a feasible solution of (P), then $\arcvalobj{2}{x^{*}}\in [\beta;\alpha]$, meaning that $\arcvalobj{2}{x^{*}}\geq \beta$.
    Hence, we can deduce $\arcvalobj{1}{x^{*}}\leq \frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot \arcvalobj{2}{x^{*}}}{\delta_{1}}\leq \frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot \beta}{\delta_{1}}$, i.e., $\arcvalobj{1}{x^{*}}\leq \bsupvalobj{1}{x_{1}}{\delta}$.
\end{proof}

\textbf{Property \ref{pte:graphs_twophases:valid_upper_bound2}} provides an upper bound that can be computed independently from the values $\arcvalobj{1}{x^{*}}$ and $\arcvalobj{2}{x^{*}}$.
Besides, we can also prove that for any $R\neq \beta$, the bound would be either looser or invalid.


\vspace{2mm}
\begin{pte}
    \label{pte:graphs_twophases:best_R}
    Let $(x_{1},x_{2})$ be a pair of consecutive solutions in $S$.
    Let $\delta$ be such that $\agg{\delta}{x_{1}}=\agg{\delta}{x_{2}}$.
    For any $R\leq\beta$, $\bsupvalobj{1}{x_{1}}{\delta}\leq \frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot R}{\delta_{1}}$.
    For any $R>\beta$, $\frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot R}{\delta_{1}}$ is not a valid upper bound for the value of the optimal solution $\arcvalobj{1}{x^{*}}$ of (P)
\end{pte}
\begin{proof}
    Clearly, for any $R\leq\beta$, $\frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot \beta}{\delta_{1}}\leq \frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot R}{\delta_{1}}$.
    Consider the case $R>\beta$.
    As $\arcvalobj{2}{x^{*}}\geq \beta$, there is no guarantee that $R \leq \arcvalobj{2}{x^{*}}$.
    Hence, it is not possible to deduce $\arcvalobj{1}{x^{*}}\leq \frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot R}{\delta_{1}}$ as done in \textbf{Property \ref{pte:graphs_twophases:valid_upper_bound2}}.
    The following \textbf{Example \ref{ex:graphs_twophases:counter_example}} gives a counter-example to complete this proof in the case $R>\beta$.
\end{proof}


\color{AH}

\vspace{2mm}
\begin{example}
    \label{ex:graphs_twophases:counter_example}
    
    Consider problem (P) with no additional constraints besides the main one, with bounds $\beta=3$ and $\alpha =5$.
    Consider this problem to have three distinct solutions denoted $x_{1}$, $x_{2}$ and $x_{3}$ with the following values: $(7,1), (5-\epsilon,3)$ where $5 - \epsilon < 4$ and, $(2,6)$, respectively. %$\arcvalobj{1}{x_{1}}=7$, $\arcvalobj{2}{x_{1}}=1$, $\arcvalobj{1}{x_{2}}=5-\epsilon<4$, $\arcvalobj{2}{x_{2}}=3$ and $\arcvalobj{1}{x_{3}}=2$, $\arcvalobj{2}{x_{3}}=6$\PB{, respectively}.
    Note that we are in the case LID.
    Indeed, the optimal solution $x_{SP}^{*}$ of the sub-problem (SP) is $x_{1}$, as $\arcvalobj{1}{x_{1}}>\arcvalobj{1}{x_{2}}>\arcvalobj{1}{x_{3}}$ and $\arcvalobj{2}{x_{1}}=1<\beta=3$.
    
    Consider now the bi-objective relaxation problem (BOR) associated with (P).
    All the following explanations are illustrated in Figure \ref{fig:counter_example}.
    
    Clearly, solutions $x_{1}$ and $x_{3}$ are Pareto-supported, but not $x_{2}$.
    Hence, the list of Pareto-supported solutions $S$ is $\{x_{3}, x_{1}\}$.
    Due to bounds $\alpha$ and $\beta$, only $x_2$ is a feasible solution of (P), meaning $x_2$ is the optimal one.

    Consider vector $\delta=(1, 1)$  such that $\agg{\delta}{x_{1}}=\agg{\delta}{x_{3}}$.
    Let $R$ be any number such that $R>\beta$.
    For any value $R$, $\frac{\agg{\delta}{x_{1}}-\delta_{2}\cdot R}{\delta_{1}}=\frac{1 \cdot 7 + 1 \cdot 1 - 1 \cdot R}{1} = 8-R$.
    As $R>\beta=3$, we deduce $8-R<5$.
    For this instance, one can select $\epsilon< R-5$ such that $\arcvalobj{1}{x_{2}} = 5-\epsilon>8 - R$.
    Consequently, if $R>\beta$, one cannot deduce a valid upper bound for the value $\arcvalobj{1}{x^{*}}$ of the optimal solution of (P).
\end{example}

\begin{figure}[htb!]
    \centering
    \includegraphics{figures/figure_counter_example.pdf}
    \caption{Illustration for Example \ref{ex:graphs_twophases:counter_example}}
    \label{fig:counter_example}
\end{figure}

\color{black}

From the previous \textbf{Properties \ref{pte:graphs_twophases:valid_upper_bound2}} and \textbf{\ref{pte:graphs_twophases:best_R}}, we know that for a given pair $(x_{1},x_{2})$ of consecutive solutions in $S$, there is no $R\neq \beta$ providing a tighter upper bound computed as $\bsupvalobj{1}{x_{1}}{\delta}$.
Recall that the number of Pareto-supported solutions can be exponential, hence one needs to compute an exponential number of bounds.
We prove in the following that it is also possible to identify the pair $(x_{1},x_{2})$ of consecutive solutions in $S$ that provides the tightest bound $\bsupvalobj{1}{x_{1}}{\delta}$.

\vspace{2mm}
\begin{thm}
    \label{thm:graphs_twophases:best_upper_bound}
    Let $(x_{1},x_{2})$ be a pair of consecutive solutions in $S$ such that $\arcvalobj{2}{x_{1}}\geq \beta>\arcvalobj{2}{x_{2}}$.
    Let $\delta$ be such that $\agg{\delta}{x_{1}}=\agg{\delta}{x_{2}}$.
    Solution $x_{1}$ and vector $\delta$ minimize the value $\bsupvalobj{1}{x_{1}}{\delta}$.
\end{thm}

\color{AH}
The proof of \textbf{Theorem \ref{thm:graphs_twophases:best_upper_bound}} is in \textbf{Appendix \ref{anx:graphs_twophases:best_upper_bound}}

Recall that the case LID is considered in this section.
Hence, \textbf{Theorem \ref{thm:graphs_twophases:best_upper_bound}} directly applies. 
Note that in the LIE case, \textbf{Theorem \ref{thm:graphs_twophases:best_upper_bound}} can also apply by considering an \textit{inverted bi-objective relaxation} of $(P)$, where $(BOR)$ maximizes $(cx, -\gamma x)$.
Results from \textbf{Properties \ref{pte:graphs_twophases:trivial_bound}} and \textbf{\ref{pte:graphs_twophases:valid_upper_bound1}} as well as \textbf{Corollary \ref{crl:graphs_twophases:valid_upper_bound1}} hold for the inverted bi-objective relaxation.
Results from \textbf{Property \ref{pte:graphs_twophases:valid_upper_bound2}} can be adapted.
To do so, we introduce $\bsupvalobjinv{1}{x_{1}}{\delta}$, which is similar to $\bsupvalobj{1}{x}{\delta}$, but with $-\alpha$ instead of $\beta$.
Similarly, \textbf{Property \ref{pte:graphs_twophases:best_R}} and \textbf{Theorem \ref{thm:graphs_twophases:best_upper_bound}} can both be adapted by considering $-\alpha$ instead of $\beta$.

In the case LF, it is not possible to infer a better bound than $\arcvalobj{1}{x_{SP}^{*}}$, with $x_{SP}^{*}$ the optimal solution of sub-problem (SP).
Indeed, in the case LF, solution $x_{SP}^{*}$ satisfies bounds $\beta$ and $\alpha$, hence might be the optimal solution to (P) provided it is feasible with respect to all additional constraints.
Any tighter bound than $\arcvalobj{1}{x_{SP}^{*}}$ would discard this solution.
Consequently, the tightest bound $\bsupvalobj{1}{x_{SP}^{*}}{\delta}$ is obtained with $\delta=(1, 0)$.
\color{black}


\subsection{Algorithm of Phase I}
\label{sec:exfirstphase}


\color{AH}
The aim of this first phase is to provide upper bounds to define a search space for the second phase of the BORWin algorithm.
More precisely, in this first phase we search for a Pareto-supported solution $x_{1}$, as well as a vector $\delta$ that can provide the tightest bound $\bsupvalobj{1}{x_{1}}{\delta}$ for the value of the optimal solution $x^{*}$ of (P).
The first step is then to identify if problem (P) is in the case LIE, LID or LF.
To do so, one needs $x_{SP}^{*}$ the optimal solution of (SP) and compare $\arcvalobj{2}{x_{SP}^{*}}$ to the bounds $\beta$ and $\alpha$.
In case LF, the algorithm stops and returns $x_{SP}^{*}$ and $\delta=(1, 0)$.
In case LID (resp. LIE), we consider (BOR), the (resp. inverted) Bi-Objective Relaxation of (P).
From Theorem \ref{thm:graphs_twophases:best_upper_bound}, one needs to find
$(x_{1},x_{2})$ a pair of consecutive solutions in $S$ such that $\arcvalobj{2}{x_{1}}\geq \beta>\arcvalobj{2}{x_{2}}$ in case LID or  $\arcvalobj{2}{x_{1}}\geq - \alpha>\arcvalobj{2}{x_{2}}$ in case LIE.

The idea to obtain this pair of solutions is to do an enumeration of Pareto-supported solutions following the dichotomic principle.
We detail the method only for the LID case, as the LIE case is similar, but with bound $-\alpha$ instead of $\beta$.
The steps of this enumeration are illustrated in Figure \ref{fig:first_phase}, where $\delta_{i,j}$ denotes a vector such that $\agg{\delta_{i,j}}{x_{i}} = \agg{\delta_{i,j}}{x_{j}}$.
We start with two Pareto-supported solutions $x_{1}$ and $x_{2}$, not necessarily successive in $S$, such that $\arcvalobj{2}{x_{1}}\geq \beta>\arcvalobj{2}{x_{2}}$ as represented in Figure \ref{fig:first_phase_a}.
Let $\delta$ be such that $\agg{\delta}{x_{1}} = \agg{\delta}{x_{2}}$.
From there, we distinguish two cases.

The first case is if the solution $x_{3}$ maximizing $\agg{\delta}{x_{3}}$ is such that $x_{3} \paretoeq{} x_{1}$ or $x_{3} \paretoeq{} x_{2}$.
Then, we know from Corollary \ref{crl:graphs_twophases:valid_upper_bound1}, that $x_{1}$ and $x_{2}$ are successive in $S$.
As such, we can return $x_{1}$ and $\delta$, as we found $(x_{1},x_{2})$ a pair of consecutive Pareto-supported solutions in $S$ such that $\arcvalobj{2}{x_{1}}\geq \beta>\arcvalobj{2}{x_{2}}$.

The second case is if the solution $x_{3}$ maximizing $\agg{\delta}{x_{3}}$ is such that $x_{3} \paretoneq{} x_{1}$ and $x_{3} \paretoneq{} x_{2}$.
Then, we know from Corollary \ref{crl:graphs_twophases:valid_upper_bound1}, that  $\arcvalobj{1}{x_{3}} \in ]\arcvalobj{1}{x_{1}};\arcvalobj{1}{x_{2}}[$ and $\arcvalobj{2}{x_{3}} \in ]\arcvalobj{2}{x_{2}};\arcvalobj{2}{x_{1}}[$.
In other words, $x_{3}$ is a Pareto-supported solution between $x_{1}$ and $x_{2}$ in $S$.
If $\arcvalobj{2}{x_{3}}\geq \beta$, then one can consider the two solutions $x_{3}$ and $x_{2}$ rather than $x_{1}$ and $x_{2}$ as shown in Figure \ref{fig:first_phase_b}.
Otherwise, one can consider the two solutions $x_{1}$ and $x_{3}$ rather than $x_{1}$ and $x_{2}$.

The idea is to use this new pair, either $x_{1}$ and $x_{3}$ or $x_{2}$ and $x_{3}$, and reuse the result of Corollary \ref{crl:graphs_twophases:valid_upper_bound1} \sout{to either} either to prove \sout{the two} both solutions to be successive in $S$, or to find a new solution $x_{4}$.
Figure $\ref{fig:first_phase_c}$ and $\ref{fig:first_phase_d}$ show an example of solution $x_{4}$ and $x_{5}$ obtained by this method.

\begin{figure}[htb!]
    \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figure_example_first_phase_a.pdf}
    \caption{First two solutions}
    \label{fig:first_phase_a}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figure_example_first_phase_b.pdf}
    \caption{Third solution}
    \label{fig:first_phase_b}
    \end{subfigure}
    
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figure_example_first_phase_c.pdf}
    \caption{Fourth solution}
    \label{fig:first_phase_c}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figure_example_first_phase_d.pdf}
    \caption{Fifth solution}
    \label{fig:first_phase_d}
    \end{subfigure}
    \caption{\AH{Illustrations of the dichotomic enumeration of the first phase}}
    \label{fig:first_phase}
\end{figure}

Algorithm \ref{alg:graphs_twophases:first_phase} gives a pseudo-code for this first phase.
Lines 1 to 10 identify the applicable case among LF, LID or LIE.
In the case LF, it returns the solution $x_{SP}^{*}$ with vector $\delta=(1, 0)$ (line 3).
Lines 11 and 13 define the first two solutions.
In this case the solutions maximizing respectively the first and the second objective are sected.
In the case where the solution maximizing the second objective has the second objective smaller than the lower bound $\beta$, then clearly no solution of (P) will satisfy this bound, hence the algorithm stops (line 14 and 15).
Lines 17 to 26 are the while loop to enumerate until the new solution is Pareto-equal to the two incumbent solutions.
The vector used to compute the new solution is at line 23, and the new solution is obtained at line 24.
At line 25 the algorithm returns one of the two incumbent solutions as well as the vector $\delta$ used in the while loop.

\begin{algorithm}[!htb]
\caption{BORWin: first phase}\label{alg:graphs_twophases:first_phase}
\begin{algorithmic}[1]
\Require A MIP of the form of (P)
\State Compute $x_{SP}^{*}$ the optimal solution of (SP)
\If{$\arcvalobj{2}{x_{SP}^{*}}\in [\beta;\alpha]$}
    \State \Return $x_{SP}^{*}$, \PB{$\delta=(1, 0)$}
\EndIf
\State $caseLIE\gets False$, $caseLID \gets False$
\If{$\arcvalobj{2}{x_{SP}^{*}}<\beta$}
    \State Define (BOR) as the Bi-Objective relaxation of (P)
    \State $caseLID \gets True$
\Else
    \State Define (BOR) as the inverted Bi-Objective relaxation of (P)
    \State $caseLIE \gets True$
\EndIf
\State $x_{A}=x_{SP}^{*}$
\State $\delta \gets$ \PB{$(0,1)$}
\State $x_{B} \gets$ solution of (BOR) maximizing $\agg{\delta}{x_{B}}$
\If{$\arcvalobj{2}{x_{B}}<\beta$}
    \State No feasible solution to (P)
    \State \CR{\Return Infeasible}
\EndIf
\State $x_{C}\gets \emptyset$
\While{$x_{C} \paretoneq{} x_{A}$ and $x_{C} \paretoneq{} x_{B}$}
    \If{$C_{C}\neq \emptyset$}
        \If{$caseLID$ and $\arcvalobj{2}{x_{C}}> \beta$}
            \State $x_{B}\gets x_{C}$
        \ElsIf{$caseLIE$ and $\arcvalobj{2}{x_{C}}> -\alpha$}
            \State $x_{B}\gets x_{C}$
        \Else
            \State $x_{A} \gets x_{C}$
        \EndIf
    \EndIf
    \State $\delta\gets$\PB{$\left( 1,\frac{\arcvalobj{1}{x_{A}}-\arcvalobj{1}{x_{B}}}{\arcvalobj{2}{x_{B}}-\arcvalobj{2}{x_{A}}}\right)$} 
    \State Compute $x_{C} \gets $ solution of (BOR) maximizing $\agg{\delta}{x_{C}}$
\EndWhile
\State \Return $x_{A}$, $\delta$
\end{algorithmic}
\end{algorithm}


\color{AH}

With a solution $x$ and a vector $\delta$ obtained from \textbf{Algorithm \ref{alg:graphs_twophases:first_phase}}, we can define a search space for the second phase.
To do so, we use four valid bounds for the optimal solution $x^{*}$ of $P$.
Clearly, $x^{*}$ is a valid solution of $P$, hence $\beta \leq \arcvalobj{2}{x^{*}}\leq \alpha$.
Then, as shown in \textbf{Property \ref{pte:graphs_twophases:valid_upper_bound2}} $\arcvalobj{1}{x^{*}} \leq \bsupvalobj{1}{x}{\delta}$.
Finally, $\agg{\delta}{x^{*}} \leq \agg{\delta}{x}$, otherwise there would be a contradiction with the definition of \textbf{Algorithm \ref{alg:graphs_twophases:first_phase}}.
The following example illustrates how these bounds are used to define a search space.


\begin{example}
Consider three instances of problem $P$, each with five solutions, $x_{1}, \ldots, x_{5}$.
For each instance, solution $x_{4}$ is with the highest value.
The first instance is in the case LID, i.e., $\arcvalobj{2}{x_{4}} < \beta$.
The second instance is in the case LF, i.e., $\arcvalobj{2}{x_{4}} \in [\beta; \alpha]$.
The third instance is in the case LIE, i.e., $\arcvalobj{2}{x_{4}} > \alpha$.
\textbf{Figures \ref{fig:obj_space_1}}, \textbf{\ref{fig:obj_space_2}} and \textbf{\ref{fig:obj_space_3}} show the search space in grey, for the first, second and third instance, with a bi-objective relaxation.
\textbf{Figures \ref{fig:obj_space_4}} shows the search space in grey for the third instance, with an inverted bi-objective relaxation.
It appears that the search space is reduced when using an inverted bi-objective relaxation in case LIE.
    
\end{example}

\begin{figure}[htb!]
    \centering
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/obj_space_1.pdf}
    \caption{Case LID}
    \label{fig:obj_space_1}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/obj_space_2.pdf}
    \caption{Case LF}
    \label{fig:obj_space_2}
    \end{subfigure}
    
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/obj_space_3.pdf}
    \caption{Case LIE}
    \label{fig:obj_space_3}
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/obj_space_4.pdf}
    \caption{Case LIE with inverted bi-objective relaxation}
    \label{fig:obj_space_4}
    \end{subfigure}
    \caption{\AH{Representation of each path of the BOLPP in the objective space}}

    \label{fig:obj_space}
\end{figure}

\color{CR}
\subsection{Relationship to Lagrangian and Dantzig-Wolfe relaxation}

The first phase of the BORWin algorithm, described in Section \ref{sec:exfirstphase}, can be shown to return the optimal solution of the lagrangian relaxation of $(R)$.

Indeed, suppose we dualize constraint \eqref{borne_min_ressource}, we obtain Lagrangian function $\theta$ defined for $\lambda \geq 0$:
$$
\theta(\lambda) = \max_{x \in X} cx + \lambda (\beta - \gamma x ) 
$$

We consider the Lagrangian minimization problem
    \begin{alignat}{3}
   \min_{\lambda \geq 0} \theta(\lambda) =  \quad & \underset{\sigma, \lambda} {\text{min}}
    & & \sigma + \lambda \beta \nonumber \\
    & \text{s. t.} \quad
    & & \sigma \geq c - \lambda \gamma x_k & & \quad \forall k \in \{1, ..., K\}\\
    &&& \lambda \geq 0
\end{alignat}
    an optimal solution $\lambda^*=\arg\min_{\mu \geq 0} \theta(\lambda) $
    and its linear programming dual, namely the Dantzig-Wolfe relaxation:
\begin{alignat}{3}
     (DW) \quad & \underset{\pi} {\text{max}}
    & & \sum_{k=1}^K (c x_k) \pi_k \nonumber \\
    & \text{s. t.} \quad
    & & \sum_{k = 1 }^K \pi_k =1 \label{convexite} \\
    &&& \beta \leq  \sum_{k=1}^K \pi_k \gamma (x_k  ) \label{ressource_dualisee} \\
    &&& \pi_k \in [0,1] & & \forall k \nonumber
\end{alignat}
where $\mbox{Ext}($X$) = \{x_1, ..., x_K\}$ is the set of extreme points of $X$.

First we give a practical lemma on the solution structure of $(DW)$ relying on the fact that only one constraint is dualized.

\begin{lem}
\label{lem:opt_dw}
There exists an optimal solution $\pi^*$ of $(DW)$ such that : $\exists i, j \in [K]$ verifying
\begin{itemize}
    \item  $\pi^*_k = 0 \quad \forall k \not=i, j$
    \item $\pi_i + \pi_j = 1$
    \item $\pi_i (\gamma x_i) + \pi_j (\gamma x_j) = \beta$
    \item The value $v^* = \pi_i (c x_i) + \pi_j (c x_j) = \theta(\lambda^*)$ is an upper bound on the value of $(P)$
\end{itemize}
\end{lem}
\begin{proof}
    The optimal solution $\pi^*$ of this relaxation corresponds to a convex combination of extreme points of $X$ that maximizes the value $\sum_{k=1}^K (c x_k) \pi_k $ while ensuring the minimum resource bound $\beta$.
    
    Since there is only one dualized constraint, we can geometrically represent the solutions of problem $(R)$ in 2 dimensions, in the space (value $v=cx$, resource $r=\gamma x$).
    
    We consider the convex hull $H$ of the extreme points of $X$ in the 2-dimensional space (v,r).
In this space, the feasible set $F$ of $(DW)$ corresponds to the intersection of $H$ with the half-space of equation ``$r \geq \beta$".

The optimal point of $(DW)$ will therefore correspond to the extreme point of $H$ that maximizes the value $v$. This point is at the intersection of the line ``$r=\beta$" (because we are in the LID case) and a facet of $H$, defined by a segment between two extreme points $x_i$ and $x_j$ of the hull $H$ (because we are in a 2-dimensional space).

\end{proof}
We denote  $\widetilde{x}_1$ and $\widetilde{x}_2$ the two extreme points with non-zero support in $\pi^*$.

In the following, we prove that the coefficients $\delta$ obtained at convergence of Phase I correspond to an optimal solution $\lambda^*$ of the Lagrangian minimization problem.
Moreover, $\widetilde{x}_1$ and $\widetilde{x}_2$ are optimal solutions of $(BOR)$ maximizing $\mu_{\delta}$.

\begin{pte}\label{prop:equiv-LR}
Let $(x_A, \delta=(1, \delta_2))$ be the result obtained at convergence of Algorithm \ref{alg:graphs_twophases:first_phase} (when not infeasible). Then, $\mu_\delta (\widetilde{x}_1) = \mu_\delta (\widetilde{x}_2) = \mu_\delta (x_A) $. 
Moreover, there exists $\lambda^* \in \arg\max \theta(\lambda)$ such that $\delta = (1, \lambda^*)$.
\end{pte}


\begin{proof}



%Note that $ \theta(\mu)$ is an upper bound on the value of $(P)$, and the minimization seeks a $\mu^*$ that minimizes this bound. Let $x^*$ be the optimal $x$ associated, $i.e.$, $x^* =\arg\max_{x \in X} cx + \mu^* (\beta - \gamma x )$. $$\theta(\mu^*) = v^* + \mu^* (\beta - r^*) \qquad \mbox{where} \quad v^* = c x^*, \quad r^* = \gamma x^*$$


%In this space, optimal solution $(\mu^*, x^*)$ defines a line with equation $\theta(\mu^*) = v + \mu^* (\beta - r)$ passing through the point $x^* = (v^*, r^*)$ and such that the upper bound $\theta(\mu^*)$ on the value of $(P)$ is obtained for $r = \beta$.


Note that the goal of Algorithm \ref{alg:graphs_twophases:first_phase}  is precisely to find a pair of points $x_A \in X$ and $x_B \in X$ such that:
\begin{itemize}
  \item Solutions $x_A$ and $x_B$ are Pareto-supported (thus are extreme points of the convex hull $H$)
  \item Solutions $x_A$ and $x_B$ are consecutive in the ordered set of supported-Pareto points $S$ (therefore the segment between $x_A$ and $x_B$ is a facet of $H$)

  \item Consider the line equation with equation $\theta = v + \lambda( \beta - r)$ passing through $x_A$ and $x_B$ ($\theta$ and $\lambda$ being determined by this condition). Solutions $x_A$ and $x_B$ are such that $\theta$ is minimal among pairs satisfying the above two properties.
\end{itemize}

Thus, we can conclude that solutions  $\widetilde{x}_1$, $\widetilde{x}_2$, $x_A$ and $x_B$ are all on the same line $\theta = v + \lambda( \beta - r)$, using Lemma \ref{lem:opt_dw}.
This line has slope $-\delta_2$, as $\delta_2= \frac{\arcvalobj{1}{x_{A}}-\arcvalobj{1}{x_{B}}}{\arcvalobj{2}{x_{B}}-\arcvalobj{2}{x_{A}}}$.
Therefore, $\mu_\delta (\widetilde{x}_1) = \mu_\delta (\widetilde{x}_2) = \mu_\delta (x_A) $.

There  exists $\lambda^* \in \arg\max \theta(\lambda)$ such that the slope of this line is also equal to $-\lambda^*$: indeed, if the resource $\beta$ decreases by one unit, a new optimal solution of $(DW)$ can be found on the line between $\widetilde{x}_1$ and $\widetilde{x}_2$, with increased objective value corresponding to an optimal dual value of constraint \eqref{ressource_dualisee}.
\end{proof}

\color{black}


\section{Phase II of the BORWin algorithm: %an 
a label-extension procedure for the ARWLPP}
\label{sec:borwin}

We consider now the ARWLPP from node $s$ to node $p$ in acyclic graph $G=(V,A)$, as described in sections \ref{sec:RWSPP} and \ref{sec:RWLPP}. Recall that the ARWLPP aims at finding a path $C=(V_C,A_C)\in{\cal C}_{sp}$  of maximal value $V(C)$ in the acyclic graph $G=(V,A)$, while satisfying all resource window constraints, i.e. $\underline{R}_u \leq R(C_{su}) \leq \overline{R}_u$, $\forall u\in V_C$.
For the first phase, we identify $V_1(C)=V(C)=\sum_{a\in A_C} V(a)$ as the value of a path $C\in{\cal C}_{sp}$ and $V_2(C)=R(C)=\sum_{a\in A_C} R(a)$ as its used resource amount.
The second phase of the BORWin algorithm aims at solving the ARWLPP.
During the first phase, Algorithm \ref{alg:graphs_twophases:first_phase} defined a region where the ARWLPP optimum lies.
Then, the second phase aims to enumerate the solutions inside this region, until the optimal solution of the ARWLPP is found and proven optimal.
In the following, let $\delta$ be the vector obtained from the first phase \CA{by ignoring all resource-window constraint except the one on node $p$}.
The aim of the second phase is to enumerate the solutions of the search space defined from the first phase.
To do so, we implicitly enumerate paths of the ABOLPP with \CA{a label extension} algorithm 
for the LPP problem with objective $\agg{\delta}{.}$ \CA{using the direction $\delta$ both to guide the search and to prune partial paths such as in lagrangian relaxation-based label extension algorithms for the RCSPP \cite{dumitrescu2003improved}}.

%variant of the $K$-best paths algorithm \cite{lawler1972procedure} 

These paths are progressively modified in order to build feasible paths of the ARWLPP that lie in the search space.
In order to make such progressive modifications, we introduce  the concept of hybrid paths and establish properties on which the algorithm efficiency relies in section \ref{sec:hybridpaths}. 
We also provide in section \ref{sec:UB-mutichoiceknapsack} an additional upper bounding scheme when the ARWLPP has the special structure of a multiple choice knapsack with nested resource window constraints.
The overall second-phase algorithm is described in section \ref{sec:secondphasealg}.

\subsection{Properties of hybrid paths and dominance rule}
\label{sec:hybridpaths}

\begin{dfn}[Hybrid path $H$]
    A hybrid path $H$ \CA{in graph $G=(V,A)$} is composed of two sub-paths:
    $H_{RW}$ from $s$ to a vertex $v$, and $H_{BO}$ from $v$ to $p$.
    Sub-path $H_{RW}$ satisfies the resource windows of the RWLPP, while $H_{BO}$ relaxes them.
\end{dfn}

From such hybrid paths, it is possible to define upper bounds of value $\agg{\delta}{C}$ for any path $C$ feasible for the RWLPP.


\vspace{2mm}
\begin{thm}\label{thm:ub:borwin2}
    Let $H=(H_{RW},H_{BO})$ be a hybrid path from $s$ to $p$, with $H_{BO}$ maximizing $\agg{\delta}{H_{BO}}$.
    For any path $C$ from $s$ to $p$ feasible for the RWLPP, starting with $H_{RW}$, then $\agg{\delta}{H}\geq \agg{\delta}{C}$.
\end{thm}
\begin{proof}
    By definition, $H_{RW}$ is a path from $s$ to a vertex $v$, and $H_{BO}$ is from $v$ to $p$.
    As $C$ starts with $H_{RW}$, then it can be decomposed as follows: $C=(H_{RW},C')$, with $C'$ from $v$ to $p$.

    Suppose $\agg{\delta}{H}<\agg{\delta}{C}$, then as $H=(H_{RW},H_{BO})$ and $C=(H_{RW},C')$, we deduce $\agg{\delta}{H_{BO}}<\agg{\delta}{C'}$.
    Recall that sub-path $H_{BO}$ relaxes the resource windows, and $C'$ takes them into account as $C$ is feasible for the RWLPP.
    Hence, there is a contradiction, $H_{BO}$ cannot maximize $\agg{\delta}{H_{BO}}$.
\end{proof}

Let $\overline{C}_v$ denote the longest path from $v$ to $p$ in $G$ according to $V(.)$ ignoring all resource window constraints and
Let $W=\sum_{a\in H_{RW}}V(a)$ the value of a feasible subpath $H_{RW}$ from $s$ to $v$.
Let $H=(H_{RW},H_{BO})$ denote an hybrid path  with  $H_{BO}$ the sub-path from node $v$ to node $p$ maximizing $$\agg{\delta}{H_{BO}}=\delta_1\sum_{a\in H_{BO}}V(a) + \left\{\begin{array}{ll}
\delta_2 \sum_{a\in H_{BO}}R(a) & (\text{LID case}: W+R(\overline{C}_v)<\beta)\\
-\delta_2 \sum_{a\in H_{BO}}R(a) & (\text{LIE case}: W+R(\overline{C}_v)>\alpha)\\
0 & (\text{LF case}: \alpha\leq W+R(\overline{C}_v)\leq \beta)
\end{array}
\right..
$$ Because of Property \ref{prop:equiv-LR} and Theorem \ref{thm:ub:borwin2}, $H_{BO}$ provides an upper bound of the cost of a feasible sub-path issued from $v$.  In the LF case, the upper bound is $W+V(\overline{C}_v)$. In the LID case the upper bound is $W+\frac{\agg{\delta}{H_{BO}}-\delta_2\beta}{\delta_1}$. In the LIF case, the upper bound is $W+\frac{\agg{\delta}{H_{BO}}+\delta_2\alpha}{\delta_1}$.

A lower bound on the value $\agg{\delta}{C^{*}}$, with $C^{*}$ the optimal path of the RWLPP can also be obtained.

\vspace{2mm}
\begin{thm}
    \label{thm:graphs_twophases:lower_bound}
    Let $C$ and $C^{*}$ be respectively a feasible and the optimal path for the RWLPP.
    Let $\underline{\agg{\delta}{C}}=\delta_{1}\cdot \arcvalobj{1}{C}+\delta_{2}\cdot \minresource{p}$ in LID and LF cases and $\underline{\agg{\delta}{C^{*}}}=\delta_{1}\cdot \arcvalobj{1}{C}+\delta_{2}\cdot -\maxresource{p}$ in LIE case.
    Then the optimal path $C^{*}$ of the RWLPP is such that $\agg{\delta}{C^{*}} \geq \underline{\agg{\delta}{C}}$.
\end{thm}
\begin{proof}
    First consider cases LID and LF, i.e., $\arcvalobj{2}{C^{*}}=\arcres{C^{*}}$.
    Clearly, $\arcvalobj{1}{C^{*}}\geq \arcvalobj{1}{C}$, $\arcvalobj{2}{C^{*}} \geq \minresource{p}$.
    Hence $\agg{\delta}{C^{*}} \geq \underline{\agg{\delta}{C}} = \delta_{1}\cdot \arcvalobj{1}{C}+\delta_{2}\cdot \minresource{p}$.

    Consider now case LIE, i.e., $\arcvalobj{2}{C^{*}}=-\arcres{C^{*}}$.
    Clearly, $\arcvalobj{1}{C^{*}}\geq \arcvalobj{1}{C}$ and $\arcvalobj{2}{C^{*}}\geq -\maxresource{p}$.
    Hence $\agg{\delta}{C^{*}} \geq \underline{\agg{\delta}{C}} = \delta_{1}\cdot \arcvalobj{1}{C}+\delta_{2}\cdot -\maxresource{p}$.
\end{proof}

Thanks to Theorems \ref{thm:ub:borwin2} and \ref{thm:graphs_twophases:lower_bound} a partial path $H_{RW}$ from $s$ to $v$ such that $\agg{\delta}{(H_{RW},H_{BO})}\geq \agg{\delta}{C}$ with $C$ a feasible solution and $H_{BO}$ a $v-p$ path that maximizes $\agg{\delta}{H_BO}$ can be discarded in an enumeration algorithm such as the one proposed in this section.

Besides this upper bound we also use a weakened variant of the RCSPP dominance rule \eqref{classic-dm}.
If two feasible partial paths $C_{su}$ and $C'_{su}$ towards the same node $u$ are such that 
\begin{equation}
V(C_{su})= V(C'_{su})\text{ and }R(C_{su})\leq R(C'_{su}) \label{borwin-dm}
\end{equation}
then $C'$ can be discarded as it cannot lead to a better solution than $C$.
%\SUN{je déplace la dominance rule ici, voir si c'est le plus pertinent} --> YES
%\begin{dfn}[Dominance rule 3]
%\label{dfn:Dominancerule3}
%    Consider two partial paths $C_{1}$ and $C_{2}$, both from the source vertex $s$ to a vertex $u$.
%    Consider the case where $\minresource{u}\leq \arcres{C_{2}}$ for all $u\in \Vpoint{}$ and $\arcres{C_{1}}\leq \arcres{C_{2}}$.
%    For any path completion $C_{3}$ from $u$ to the target vertex $p$ such that ($C_{2}, C_{3}$) form a feasible path, then ($C_{1}, C_{3}$) also form a feasible path.
%    Consequently, if $\arcval{C_{1}}\geq \arcval{C_{2}}$ then $C_{2}$ is dominated.
%\end{dfn}


\color{CR}
\subsection{Complementary upper bounds based on other underlying easily solved structures}
\label{sec:UB-mutichoiceknapsack}

Problem $(P)$ has been defined as a structured problem featuring a shortest/longest path sub-structure - represented by feasible set $X$ - coupled to resource constraints \eqref{main_additional_constraint} - \eqref{additional_constraints}.
Based on such structure, phase I of the BORWin algorithm computes a Lagrangian upper bound on a weighted combination of values $V_1$ and $V_2$.

However, other useful underlying structures may exist in $(P)$, and such structures can also be exploited to compute  upper bounds complementary to the upper bounds obtained in phase I.

Consider a subproblem $(Q)$ $\max_{x \in Y} cx $ of $(P)$, $i.e.$, the solution set $Y$ contains the feasible set of $X$ :
$$
\{ x \in X \; | \; \eqref{main_additional_constraint} -  \eqref{additional_constraints} \} \subset Y
$$

Suppose problem $(Q)$ is easily solved, in the sense that there exists a very efficient algorithm to obtain an optimal solution.
Then, BORWin algorithm can benefit from the upper bound on $(P)$ obtained by solving $(Q)$.

More precisely, we suppose that the structure of $(Q)$ is preserved by partial variable fixing, $i.e.$, for any partial solution $\overline{x}$  - defined as a dictionary containing couples (index, partial solution value for this index), problem $(Q(\overline{x}))$ remains easily solved:
	\begin{alignat*}{3}
		(Q(\overline{x})) \quad & v_Q(\overline{x}) \; = \;  \max_x cx
		& &   \\
		& \text{s. t.} \;
		  x_i = \overline{x}_i & & \quad \forall i \in \overline{x}
		\end{alignat*}


Then, phase II of BORWin algorithm can efficiently rely on the following very classical result.
\begin{pte}
Consider $v$ the value of a given feasible solution to $(P)$.
For any partial solution $\overline{x}$, if $v_Q(\overline{x}) \leq v$ then partial solution $\overline{x}$ cannot lead to a better solution than $v$ (and therefore can be ``pruned").
\end{pte}

Note that for such a bound to be complementary to the Lagrangian bound from phase I, it is necessary that feasible set $Y$ be different from $X$.

For example, set $Y$ can contain a selection of resource constraints \eqref{main_additional_constraint} -  \eqref{additional_constraints} for which efficient algorithms are known. Typically, if the union of (some) of these resource constraints feature a nested multiple-choice knapsack structure, efficient linear relaxation algorithms exist \cite{armstrong1982multiple}. Moreover, if such nested multiple-choice knapsack structure features symmetric weights, an efficient dedicated A* algorithm exists to obtain an integer optimal solution \cite{heintzmann2023efficient}.
More generally, if set $Y$ can be identified to a matroid, efficient greedy algorithms are optimal \cite{faigle2009general}.


\color{black}

\subsection{The second-phase algorithm}
\label{sec:secondphasealg}

\textbf{Algorithm \ref{alg:graphs_twophases:second_phase}} describes the enumeration of the second phase, which is as follows.
We first compute a hybrid path $H=(H_{RW},H_{BO})$ with $H_{RW}=\emptyset$ and $H_{BO}$ the optimal path for the LPP from $s$ to $p$ with objective $\agg{\delta}{.}$.
Then, we consider a list of hybrid paths, initialized as $L=[H]$.
List $L$ will be kept sorted by decreasing value $\agg{\delta}{.}$ during the whole algorithm.
As long as $L$ is not empty, we proceed with the following steps.
We select \CA{$H=(H_{RW},H_{BO})$}, the first hybrid path in $L$ at line 5.
If $H$ is feasible, we obtain a lower bound $\underline{\agg{\delta}{H}}$ on $\agg{\delta}{C^{*}}$ as proven in \textbf{Theorem \ref{thm:graphs_twophases:lower_bound}}.
\CA{If we also have specific lower bound due to the special structure of the graph as stated in Section \ref{ec:UB-mutichoiceknapsack}, we denoted as $UB(H_{RW})$ this lower bound.}
Hence, we remove from $L$ all partial paths \CA{$H'=(H_{RW}',H_{BO}')$} such that $\agg{\delta}{H'} < \underline{\agg{\delta}{H}}$ \CA{or $UB(H_{RW}')< V(H)$} at line 8.
If $H$ is not feasible, it is not feasible due to $H_{BO}$ and we extend $H_{RW}$.
Let $a=(u,v)$ be the first arc of $H_{BO}$ from $u$ to $v$.
A classical labeling extension consists of building hybrid paths $H'=(H_{RW}',H_{BO}')$ with $H'_{RW}=H_{RW}\cup \{(u,v')\}$, $v'\neq v$ and $H'_{LW}$ the optimal path for the LPP from $v'$ to $p$ considering objective function $\agg{\delta}{.}$.
In this case, we generalize this extension in order to generate more new hybrid paths and obtain feasible paths quicker.
This generalized extension described in the following corresponds to lines 10 to 20.
Let $a=(u,v)$ be any arc of $H_{BO}$.
Let $SH$ be the subset of $H_{BO}$, containing all arcs before $a$.
The extension consists of building $H'=(H_{RW}',H_{BO}')$ with $H_{RW}'=H_{RW}\cup SH \cup \{u, v'\}$ and $H'_{BO}$ the longest path for the LPP from $v'$ to $p$ with objective function $\agg{\delta}{.}$.
For each $H'$ generated in this way, if $H'_{RW}$ satisfies the resource windows, then $H'$ is added to $L$.
Otherwise, $H'$ is discarded.


\begin{algorithm}
\caption{Second phase}\label{alg:graphs_twophases:second_phase}
\begin{algorithmic}[1]
\Require An RWLPP graph $G=(V,A)$ and a vector $\delta$
\State Compute $H_{BO}$ the shortest path from $s$ to $p$ maximizing $\agg{\delta}{H_{BO}}$
\State $H \gets (\emptyset, H_{BO})$
\State $L \gets [H]$
\State $C \gets \emptyset$
\While{$L\neq \emptyset$}
    \State Select \CA{$H=(H_{RW},H_{BO})$} the first element of $L$
    \If{$H$ feasible for the RWLPP}
        \State remove $H'=(H_{RW}',H_{BO}')$ from $L$ such that $\agg{\delta}{H'}< \underline{\agg{\delta}{H}}$ \CA{or $UB(H_{RW}')<V(H)$}
        \If{$C = \emptyset$ or $\arcvalobj{1}{H}>\arcvalobj{1}{C}$}
            \State $C \gets H$
        \EndIf
    \Else
        \For{$k$ in $[0; |H_{BO}|-1]$}
            \State get $SH$ the $k$ first arcs of $H_{BO}$
            \State get $a=(u,v)$ the $k+1^{\text{th}}$ arc of $H_{BO}$
            \For{arc $a'=(u,v')\in A$, $v'\neq v$}
                \State $H_{RW}'=H_{RW}\cup SH\cup a'$
                \CA{\If{$H_{BO}(v')=\emptyset$ } 
                    \State compute $H_{BO}'$ the path from $v'$ to $p$ maximizing $\agg{\delta}{H_{BO}'}$ \State Store it in $H_{BO}(v')$
                \EndIf}
                \If{$\agg{\delta}{H}\geq \underline{\agg{\delta}{C}}$ \CA{and $UB(H_{RW}')\geq V(C)$}}
                    \State add $H$ to $L$ while keeping $L$ sorted by decreasing $\agg{\delta}{.}$
                \EndIf
            \EndFor
        \EndFor
    \EndIf
\EndWhile
\State \Return $C$
\end{algorithmic}
\end{algorithm}

\color{AH}

\begin{example}
Consider the RWLPP instance described in \textbf{Example \ref{ex:RWLPP}, illustrated in \textbf{Figure \ref{fig:RWLPP}}}.
After the first phase, we obtain solution $C=(s, 1, 3, 2, p)$ and $\delta=(1, 0.053)$.

We start the second phase with a first hybrid path $H_{1}=(\emptyset, \{(s, 1), (1, 3), (3, 2), (2, p)\})$.
We initialize a list $L=[H_{1}]$.
\textbf{Figure \ref{fig:figure_phase_two_1}} gives the search space and known solution at the start of the second phase.

Hybrid path $H_{1}$ is infeasible, it satisfies all windows but the one of $p$.
Indeed, $H_{1}$ uses 35 amount of resources and $\maxresource{p}=29$.
We then remove $H_{1}$ from $L$ and create new hybrid paths from $H_{1}$.
\begin{itemize}
    \item The only arc starting with $s$, different than $(s, 1)$ is $(s, 3)$.
    The shortest path from $3$ to $p$ with vector $\delta=(1, 0.053)$ is $\{(3, p)\}$.
    Hence we have $H_{2} = (\{(s, 3)\}, \{(3, p)\})$ with $\arcvalobj{1}{H_{2}}=27$ and $\arcvalobj{2}{H_{2}}=21$.
    \item The only arc starting with $1$, different than $(1, 3)$ is $(1, 2)$.
    The shortest path from $2$ to $p$ with vector $\delta=(1, 0.053)$ is $\{(2, p)\}$.
    Hence we have $H_{3} = (\{(s, 1), (1, 2)\}, \{(2, p)\})$ with $\arcvalobj{1}{H_{3}}=29$ and $\arcvalobj{2}{H_{3}}=25$.
    \item The only arc starting with $3$, different than $(3, 2)$ is $(3, p)$.
    As $p$ is the target node, we have $H_{4} = (\{(s, 1), (1, 3), (3,p)\}, \emptyset)$ with $\arcvalobj{1}{H_{4}}=33$ and $\arcvalobj{4}{H_{4}}=16$.
    However, the part $H_{RW}$ of $H_{4}$ does not satisfy the constraints.
    Indeed, this path uses 33 amount of resources from $s$ to $p$ and $\maxresource{p}=29$.
    Consequently, we discard path $H_{4}$.
    \item There are no arc starting with $2$ different than $(2, p)$.
\end{itemize}
Two hybrid paths were generated from $H_{1}$, namely $H_{2}$ and $H_{3}$.
By adding these hybrid paths to $L$ by decreasing value $\agg{\delta}{.}$, we have $L= [H_{3}, H_{2}]$.
\textbf{Figure \ref{fig:figure_phase_two_1}} gives the search space and known solutions after the first iteration of the second phase.

Hybrid path $H_{3}$ is a feasible solution.
We save $H_{3}$ as the current best solution found and remove $H_{3}$ from $L$.
We deduce the lower bound $\underline{\agg{\delta}{H_{3}}}=\delta_{1}\cdot \arcvalobj{1}{H_{3}}+\delta_{2}\cdot \minresource{p}=30.06$.
As $\agg{\delta}{H_{2}} = 28.11 < \underline{\agg{\delta}{H_{3}}}$, we can discard solution $H_{2}$.
As such, the list $L$ is now empty, and the algorithm stops.
The algorithm returns the path corresponding to $H_{3}$ as the optimal solution.

\end{example}
\begin{figure}[htb!]
    \centering
    \begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figure_phase_two_1.pdf}
    \caption{Initial seach space for the second phase}
    \label{fig:figure_phase_two_1}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/figure_phase_two_2.pdf}
    \caption{Search space after the first iteration}
    \label{fig:figure_phase_two_2}
    \end{subfigure}
\end{figure}

%Peut-être présenter ici les idées génériques de "Further improvements" (heuristique optimiste, règles de dominance, etc...) et les détailler en seciton 5 pour le HUC?

\color{black}

%\paragraph{Further improvements.}
%Note that this second phase can be further improved.
%In the following, we present three improvements that speed-up the algorithm for the HUC problem.

%A first improvement is in the case there exists an upper bound $h_{1}(C)$ for the value $\arcvalobj{1}{C}$ of a feasible path.
%As soon as a feasible path $C$ for the RWLPP is found, we can remove from $L$ all hybrid path $H$ for which $h_{1}(H)<\arcvalobj{1}{C}$.
%In the case of the HUC problem, such upper bound have been defined in \cite{heintzmann2023efficient}, for the purpose of a variant of the A* algorithm dedicated to the HUC problem.

The second improvement is to use a classical dominance rule for the RCSPP at each vertex.
Let $H_{RW}$ be a partial path from $s$ to $v$.
Any partial path $H_{RW}'$ from $s$ to $v$ such that $\arcvalobj{2}{H_{RW}'}=\arcvalobj{2}{H_{RW}}$ and $\arcvalobj{1}{H_{RW}'}\geq \arcvalobj{1}{H_{RW}}$ cannot yield the optimal solution of the RWLPP.
Indeed, both partial path use the exact same resource, while $H_{RW}$ has a higher value.
Hence, $H_{RW}$ dominates $H_{RW}'$.
The proposed implementation is to store for each node $v$ a list containing the pairs of values $(\arcvalobj{1}{C}, \arcvalobj{2}{C})$ of all partial path enumerated from $s$ to $v$.
This implementation is particularly effective if there are many paths using the exact same amount of resource between node $s$ and a node $v$, as the lists at each vertex will remain small.
This is the case for the HUC problem, as the operating points are the same, the exact same set of water flows is used at each time period.
Note however that this implementation can produce very large lists at each node, which can slow down the BORWin algorithm for RWLPP instances for which there is no such structure for the use of the resource.

%The third improvement consists in storing the optimal solution of the LPP from any vertex $v$ to the target vertex $p$.
%Indeed, for two partial paths $H_{RW}$ and $H_{RW}'$ from $s$ to $v$, the corresponding $H_{BO}$ is the same for both.
%As such, it is possible to only compute $H_{BO}$ between $v$ to $p$ once.



